Geometry of logarithmic strain measures in solid mechanics

We consider the two logarithmic strain measures\[\omega_{\rm iso}=\|\mathrm{dev}_n\log U\|=\|\mathrm{dev}_n\log \sqrt{F^TF}\|\quad\text{ and }\quad \omega_{\rm vol}=|\mathrm{tr}(\log U)|=|\mathrm{tr}(\log\sqrt{F^TF})|\,,\]which are isotropic invariants of the Hencky strain tensor $\log U$, and show that they can be uniquely characterized by purely geometric methods based on the geodesic distance on the general linear group $\mathrm{GL}(n)$. Here, $F$ is the deformation gradient, $U=\sqrt{F^TF}$ is the right Biot-stretch tensor, $\log$ denotes the principal matrix logarithm, $\|.\|$ is the Frobenius matrix norm, $\mathrm{tr}$ is the trace operator and $\mathrm{dev}_n X$ is the $n$-dimensional deviator of $X\in\mathbb{R}^{n\times n}$. This characterization identifies the Hencky (or true) strain tensor as the natural nonlinear extension of the linear (infinitesimal) strain tensor $\varepsilon=\mathrm{sym}\nabla u$, which is the symmetric part of the displacement gradient $\nabla u$, and reveals a close geometric relation between the classical quadratic isotropic energy potential \[\mu\,\|\mathrm{dev}_n\mathrm{sym}\nabla u\|^2+\frac{\kappa}{2}\,[\mathrm{tr}(\mathrm{sym}\nabla u)]^2=\mu\,\|\mathrm{dev}_n\varepsilon\|^2+\frac{\kappa}{2}\,[\mathrm{tr}(\varepsilon)]^2\]in linear elasticity and the geometrically nonlinear quadratic isotropic Hencky energy\[\mu\,\|\mathrm{dev}_n\log U\|^2+\frac{\kappa}{2}\,[\mathrm{tr}(\log U)]^2=\mu\,\omega_{\rm iso}^2+\frac\kappa2\,\omega_{\rm vol}^2\,,\]where $\mu$ is the shear modulus and $\kappa$ denotes the bulk modulus. Our deduction involves a new fundamental logarithmic minimization property of the orthogonal polar factor $R$, where $F=R\,U$ is the polar decomposition of $F$. We also contrast our approach with prior attempts to establish the logarithmic Hencky strain tensor directly as the preferred strain tensor in nonlinear isotropic elasticity.

==> tikz/deformationDistanceExplanation.tex <==
\input{/home/bob/Desktop/svn/tex/tikz/libraries/deformationLibrary.tex}

\tikzset{curvestyle/.style={smooth, semithick, variable=\t, samples=25, domain=-1:1.75}}
\tikzset{pointNodeStyle/.style={inner sep = 0, minimum size=2, draw, circle, very thin, shade, shading=ball}}
\tikzset{textNodeStyle/.style={font = {}}}
\tikzset{tangentStyle/.style={->, semithick}}
\tikzset{arrowstyle/.style={->}}

\def\rotOut{-70}
\def\rotPhi{14}

\definecolor{Ocolor}{rgb}{.4,.4,1}
\definecolor{phiOcolor}{rgb}{1,.4,.4}
\definecolor{Otangentcolor}{rgb}{0,0,1}
\definecolor{phiOtangentcolor}{rgb}{1,0,0}

\OmegaSetDefaults
\OmegaSetGridSize{.2}{.2}
\OmegaSetOutlineSampleCount{21}
\OmegaSetGridSampleCount{12}

\OmegaSetOutlineStyle{color = darkgray, opacity = .9, thick}
\OmegaSetShadingStyle{left color = lightgray, right color = black, opacity = .15, ->}
\OmegaSetGridStyle{very thin, color=darkgray, opacity = .3}

\newcommand{\smallSquare}{%
	\OmegaSetGridStyle{opacity=0}
	\OmegaSetGridSampleCount{2}
	%
	\OmegaSetGridStyle{very thin, color=darkgray, opacity = .3}
	\OmegaSetOutlineToRectangle{-.3}{.1}{-.1}{.3}
	\OmegaDraw
}

\begin{scope}[scale=2.1,declare function ={%
		phistraightx(\x,\y)=\x;
		phistraighty(\x,\y)=1.1*\y*(1-.05*(\x)^2)-.1*(2*\x)^2-.075*(3*\x)^3;
		phix(\x,\y)=\x+.4*\y;
		phiy(\x,\y)=\y+.25*(\x+.5)^2;
		phiTwox(\x,\y)=cos(\rotPhi)*phistraightx(\x,\y) - sin(\rotPhi)*phistraighty(\x,\y);
		phiTwoy(\x,\y)=cos(\rotPhi)*phistraighty(\x,\y) + sin(\rotPhi)*phistraightx(\x,\y);
	}]

	\OmegaSetOutlineToRectangle{-.5}{-.5}{.5}{.5}

	%
	\begin{scope}
		\OmegaSetSharpOutline
		\OmegaSetDeformationToId
		\OmegaDraw

		\OmegaSetShadingStyle{left color = black, right color = black, opacity = .15, ->}
		\smallSquare
		
		\fill[color=black] (-.2,.2) circle (.01) node[above right=-1.19mm] {\footnotesize$x$};
	\end{scope}

	%
	\begin{scope}[xshift=-2.1cm, yshift=-1.4cm]
		\OmegaSetSmoothOutline
		\OmegaSetDeformation{phix}{phiy}
		\OmegaDraw

		\OmegaSetShadingStyle{left color = red, right color = red, opacity = .77, ->}
		\smallSquare
	\end{scope}

	%
	\begin{scope}[xshift=2.1cm, yshift=-1.4cm]
		\OmegaSetSmoothOutline
		\OmegaSetDeformation{phiTwox}{phiTwoy}
		\OmegaDraw

		\OmegaSetShadingStyle{left color = blue, right color = blue, opacity = .77, ->}
		\smallSquare
	\end{scope}

	%
	\begin{scope}[xshift=-1.89cm, yshift=-3.71cm]
		\OmegaSetSharpOutline
		\OmegaSetOutlineSampleCount{5}
		\OmegaSetDeformation{phix}{phiy}
		
	\begin{scope}[scale=4]
		\OmegaSetShadingStyle{left color = red, right color = red, opacity = .77, ->}
		\smallSquare
	\end{scope}
	\end{scope}

	%
	\begin{scope}[xshift=3.22cm, yshift=-3.5cm]
		\OmegaSetSharpOutline
		\OmegaSetOutlineSampleCount{5}
		\OmegaSetDeformation{phiTwox}{phiTwoy}
		
		\begin{scope}[scale=4]
			\OmegaSetShadingStyle{left color = blue, right color = blue, opacity = .77, ->}
			\smallSquare
		\end{scope}
	\end{scope}

	%
	\draw[->] (-.7,0) to[out=180, in=90] node[midway, above left]{$\varphi_1$} (-2.1,-.63);
	\draw[->] (.7,0) to[out=0, in=90] node[midway, above right]{$\varphi_2$} (2.1,-.63);

%
%

	%
	\draw[arrowstyle, <->, color=black, dashed] (-1.4,-1.4) to %
	node[midway, above]{$\mathrm{dist}(\varphi_1,\varphi_2)$} node[midway, below]{$=\int_\Omega\dg(\textcolor{red}{\grad\varphi_1(x)},\textcolor{blue}{\grad\varphi_2(x)})\,\dx$} (1.4,-1.4);
	\draw[arrowstyle, <->, color=black, dashed] (-1.4,-2.8) to %
	node[pos=.52, above=2]{$\dg(\textcolor{red}{\grad\varphi_1(x)},\textcolor{blue}{\grad\varphi_2(x)})$} (1.4,-2.8);

	%
	\node[above] at (0,.5) {$\Omega$};
\end{scope}


==> tikz/riemannianDistanceOnGLn.tex <==
%
\newcommand\pgfmathsinandcos[3]{
	\pgfmathsetmacro#1{sin(#3)}
	\pgfmathsetmacro#2{cos(#3)}
}
\newcommand\LongitudePlane[3][current plane]{
  \pgfmathsinandcos\sinEl\cosEl{#2} 
  \pgfmathsinandcos\sint\cost{#3}
  \tikzset{#1/.estyle={cm={\cost,\sint*\sinEl,0,\cosEl,(0,0)}}}
}
\newcommand\LatitudePlane[3][current plane]{
	\pgfmathsinandcos\sinEl\cosEl{#2}
	\pgfmathsinandcos\sint\cost{#3}
	\pgfmathsetmacro\yshift{\cosEl*\sint}
	\tikzset{#1/.estyle={cm={\cost,0,0,\cost*\sinEl,(0,\yshift)}}} 
}
\newcommand\DrawLongitudeCircle[2][1]{
	\LongitudePlane{\angEl}{#2}
	\tikzset{current plane/.prefix style={scale=#1}}
	\pgfmathsetmacro\angVis{atan(sin(#2)*cos(\angEl)/sin(\angEl))} 
	\draw[current plane, color=black, opacity=0.2] (\angVis:1) arc (\angVis:\angVis+180:1);
	%
}
\newcommand\DrawLatitudeCircle[2][1]{
	\LatitudePlane{\angEl}{#2}
	\tikzset{current plane/.prefix style={scale=#1}}
	\pgfmathsetmacro\sinVis{sin(#2)/cos(#2)*sin(\angEl)/cos(\angEl)}
	\pgfmathsetmacro\angVis{asin(min(1,max(\sinVis,-1)))}
	\draw[current plane, color=black, opacity=0.2] (\angVis:1) arc (\angVis:-\angVis-180:1);
	%
}
\newcommand\DrawSO[2][1]{
	\LongitudePlane{\angEl}{#2}
	\tikzset{current plane/.prefix style={scale=#1}}
	\pgfmathsetmacro\angVis{atan(sin(#2)*cos(\angEl)/sin(\angEl))} 
	\draw[current plane,color=SOcolor,opacity=1, thick] (\angVis:1) arc (\angVis:\angVis+180:1);
}
\newcommand\DrawGeodesic[4][1]{
	\LatitudePlane{\angEl}{#2}
	\tikzset{current plane/.prefix style={scale=#1}}
	\pgfmathsetmacro\sinVis{sin(#2)/cos(#2)*sin(\angEl)/cos(\angEl)}
	\pgfmathsetmacro\angStart{#3}
	\pgfmathsetmacro\angEnd{#4}
	\draw[current plane,color=GLcolor,opacity=1] (\angStart:1) arc (\angStart:-\angEnd:1);
}

\begin{scope}[]
	%
	%
	\def\uncoverGeodesicDistance{2}
	\def\uncoverEuclideanDistance{3}
	\def\uncoverTangentPlane{4}
	\def\uncoverTSO{5}
	\def\uncoverTangentDistance{6}
	%
	\definecolor{SOcolor}{rgb}{1,0,0}
	\definecolor{socolor}{rgb}{.9,0.4,0}
	\definecolor{GLcolor}{rgb}{0,0,1}
	\definecolor{glcolor}{rgb}{.5,0,1}
	\def\pointNodeSize{4}
	%
	\tikzset{pointNodeStyle/.style={inner sep = 0, minimum size=\pointNodeSize, draw, circle, very thin, shade, shading=ball}}
	\tikzset{textNodeStyle/.style={font = {}}}
	%
	\coordinate (v) at (7,-6);
	\coordinate (w) at (3,1);
	\def\lambda{.5} 
	\def\nu{1.5}
	%
	\coordinate (unity) at (0,1.785);
	\def\R{2.5}
	\def\angEl{44.5}
	
	%
	\filldraw[ball color=blue!20!green!10!,opacity=1] (0,0) circle (\R);
	\foreach \t in {-80,-70,...,80} { \DrawLatitudeCircle[\R]{\t}}
	\foreach \t in {-5,-25,...,-175} { \DrawLongitudeCircle[\R]{\t+10}}
	%
	%

	%
	\DrawSO[\R]{25}

	%
	\coordinate (F) at (1.4,-1.1){};
	\coordinate (R) at (-2.23,-.42){};
	\node[pointNodeStyle, ball color = GLcolor] (FNode) at (1.4,-1.1){};
%
		\node[pointNodeStyle, ball color = SOcolor] (RNode) at (-2.23,-.42){};
		\DrawGeodesic[\R]{10}{-56}{153.5}
%
	
	%
	\node[pointNodeStyle, ball color = black, minimum size = {1.5*\pointNodeSize}] (unityNode) at (unity){};

	%
	\node[textNodeStyle, color=SOcolor] (SOText) at (-.5,1){$\mathrm{SO}(n)$};
	\node[textNodeStyle, above left, color=black] (unityText) at (unityNode){$\id$};
%
		\node[textNodeStyle, color=SOcolor, right] (RText) at ($(R)+(0,.2)$){$R=\mathrm{polar}(F)$};
%
	
	%
%
		\draw[opacity=.75] ($(unity)-{\lambda/2}*(v)-{\nu/2}*(w)$) -- ($(unity)-{\lambda/2}*(v)+{\nu/2}*(w)$) -- ($(unity)+{\lambda/2}*(v)+{\nu/2}*(w)$) -- ($(unity)+{\lambda/2}*(v)-{\nu/2}*(w)$) -- cycle;
		\shade[ball color = blue!20!green!10!, opacity=.6] ($(unity)-{\lambda/2}*(v)-{\nu/2}*(w)$) -- ($(unity)-{\lambda/2}*(v)+{\nu/2}*(w)$) -- ($(unity)+{\lambda/2}*(v)+{\nu/2}*(w)$) -- ($(unity)+{\lambda/2}*(v)-{\nu/2}*(w)$) -- cycle;
%

	%
%
		\tikzset{connectParametersLeft/.style={semithick, color=red, opacity=.5, dotted}}
		\draw[connectParametersLeft] ($(unity)-{.2*\nu}*(w)$) -- ($(unity)-{.2*\nu}*(w)-(0,.13)$);
		\draw[connectParametersLeft] ($(unity)-{.25*\nu}*(w)$) -- ($(unity)-{.25*\nu}*(w)-(0,.22)$);
		\draw[connectParametersLeft] ($(unity)-{.3*\nu}*(w)$) -- ($(unity)-{.3*\nu}*(w)-(0,.35)$);
		\draw[connectParametersLeft] ($(unity)-{.35*\nu}*(w)$) -- ($(unity)-{.35*\nu}*(w)-(0,.49)$);
		\draw[connectParametersLeft] ($(unity)-{.4*\nu}*(w)$) -- ($(unity)-{.4*\nu}*(w)-(0,.7)$);
		\draw[connectParametersLeft, thick] ($(unity)-{.45*\nu}*(w)$) -- ($(unity)-{.45*\nu}*(w)-(0,1)$);
		%
		\tikzset{connectParametersRight/.style={thin, color=red, opacity=.7, dotted}}
		\draw[connectParametersRight] ($(unity)+{.2*\nu}*(w)$) -- ($(unity)+{.2*\nu}*(w)-(0,.14)$);
		\draw[connectParametersRight] ($(unity)+{.25*\nu}*(w)$) -- ($(unity)+{.25*\nu}*(w)-(0,.26)$);
		\draw[connectParametersRight] ($(unity)+{.3*\nu}*(w)$) -- ($(unity)+{.3*\nu}*(w)-(0,.36)$);
		\draw[connectParametersRight] ($(unity)+{.35*\nu}*(w)$) -- ($(unity)+{.35*\nu}*(w)-(0,.52)$);
		\draw[connectParametersRight] ($(unity)+{.4*\nu}*(w)$) -- ($(unity)+{.4*\nu}*(w)-(0,.72)$);
		\draw[connectParametersRight, very thin] ($(unity)+{.45*\nu}*(w)$) -- ($(unity)+{.45*\nu}*(w)-(0,1)$);
%

	%
%
		\draw[thick, color=socolor] ($(unity)-{\nu/2.1}*(w)$) -- ($(unity)+{\nu/2.1}*(w)$);
%

	%
	\coordinate (gradu) at ($(unity)+{.2*\lambda}*(v)+{.25*\nu}*(w)$){};
	\coordinate (skewgradu) at ($(unity)+{.25*\nu}*(w)$){};
%
		\node[pointNodeStyle, ball color=glcolor] (graduNode) at (gradu){};
		\draw[color=glcolor,opacity=.5,dashed,->] (unityNode) -- coordinate[midway](graduVector) (graduNode);
%
		\node[pointNodeStyle, ball color = socolor] (skewgraduNode) at (skewgradu){};
		\draw[color=glcolor,opacity=1] (graduNode) -- node[pos=.4, minimum size = 12](distglCenter){} (skewgraduNode);
		\draw[color=socolor,opacity=1,->] (unityNode) -- coordinate[midway](skewgraduVector) (skewgraduNode);
%

	%
	\def\deltaT{0.05}
	\def\minOpacity{.2}
	\def\opacityExponent{2}
	\def\maxOpacity{.7}
	\pgfmathsetmacro\opacityFactor{(\maxOpacity-\minOpacity)/pow(.5,\opacityExponent)}
%
		\foreach \t in {0,\deltaT,...,1}
			\draw[dashed, color=black, opacity={\minOpacity+\opacityFactor*pow(abs((\t+\deltaT/2)-.5),\opacityExponent)}] (${1-\t}*(F)+\t*(R)$) -- (${1-(\t+\deltaT)}*(F)+{\t+\deltaT}*(R)$);
%

	%
	%
	\node[textNodeStyle, color=black!100!blue!81!green!81] (GLText) at (-3.3,.35){$\mathrm{GL^+}(n)$};
	%
%
		\node[textNodeStyle, color=black!100!blue!81!green!81, right] (glText) at ($(unity)-{.35*\lambda}*(v)+{.5*\nu}*(w)$){$T_{\id}\mathrm{GL^+}(n)=\mathfrak{gl}(n)$};
%
		\node[textNodeStyle, color=socolor, right] (soText) at ($(unity)+{.5*\nu}*(w)$){$T_{\id}\mathrm{SO}(n)=\mathfrak{so}(n)$};
%
	%
	\node[textNodeStyle, right, color=GLcolor] (FText) at (F){$F$};
	%
%
		%
		\node[textNodeStyle, below, color=glcolor, font=\small] (graduText) at (graduVector){$\nabla u$};
%
		%
		\node[textNodeStyle, above=7, left=-9, color=socolor, font=\small] (skewgraduText) at (skewgraduVector){$\mathrm{skew}\nabla u$};
%

	%
	\tikzset{arrowstyle/.style={<-, dotted, thick}}
	\tikzset{formulastyle/.style={align=left, font={\footnotesize}}}
%
		\draw[arrowstyle, color=glcolor] (distglCenter) .. controls (3,2) and (4,1.8) .. (4.76,1.4) node[formulastyle, color=glcolor, right]{\\[7mm]$\mathrm{dist}_{\mathrm{euclid},\,\mathfrak{gl}}^2(\nabla u, \mathfrak{so}(n))$\\[1mm]$\hspace{-3mm}=\mu|\!|\mathrm{dev}_n\,\mathrm{sym} \nabla u|\!|^2 + \frac{\kappa}{n}[\mathrm{tr}\nabla u]^2$};
%
%
		\draw[arrowstyle, color=darkgray] (.1,-.7) .. controls (1,-.2) and (3,-.2) .. (4.5,-.2) node[formulastyle, color=darkgray, right]{\\[4mm]$\mathrm{dist}_{\mathrm{euclid}}^2(F, \mathrm{SO}(n))$\\[1mm] $\hspace{-3mm}=|\!|U-\id|\!|^2 = |\!|\sqrt{F^T\!F}-\id|\!|^2$};
%
		\draw[arrowstyle, color=GLcolor] (.1,-1.55) .. controls (1,-2.3) and (3,-2.3) .. (4.2,-2) node[formulastyle, color=GLcolor, right]{\\[4mm]$\mathrm{dist}_{\mathrm{geod}}^2(F, \mathrm{SO}(n))$\\[1mm] $\hspace{-3mm}=\mu|\!|\mathrm{dev}_n\,\mathrm{log}\,U|\!|^2 + \frac{\kappa}{n}[\mathrm{tr}(\mathrm{log}U)]^2$};
%
\end{scope}
